Spherical Fixed-Point Reasoners: Adaptive Loop Halting on the Hypersphere

Looped (weight-tied) transformers enable adaptive computation by allocating more iterations to harder inputs. Fixed-Point Reasoners (FPRM) achieve this with a damped fixed-point solver, but operate in an unbounded Euclidean residual space with coupled rescaling and relative-norm halting. We introduce Spherical Fixed-Point Reasoners (SFPRM), which perform the same computation on the unit hypersphere of normalized transformers (nGPT). Input injection, damping, and halting become geodesic operations, yielding boundedness by construction and eliminating coefficient coupling. We prove fixed-point existence, local convergence under an explicit step-size condition, and global convergence under strong injection. On Sudoku-Extreme, Maze-Hard, and Mini-ARC, SFPRM achieves 96.6%, 87.9%, and 59.1% test accuracy, respectively, outperforming FPRM and other baselines while allocating test-time compute more effectively. Its converged geometry is also interpretable: token-input angles capture puzzle structure and predict correctness.

==> sections/tikz_files/circle.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=1.1, >=Stealth, font=\small]
  \def\R{3.2}
  \coordinate (O) at (0,0);

  % Great-circle cross-section: the 2-plane span{u,v} in which Slerp lives.
  \draw[thick, black!55] (O) circle (\R);

  % Two unit states and the Slerp point (eta = 0.45).
  \coordinate (u) at (16:\R);
  \coordinate (v) at (76:\R);
  \coordinate (p) at (43:\R);

  % Radii to u and v.
  \draw[->, black!70] (O) -- (u);
  \draw[->, black!70] (O) -- (v);

  % Geodesic (great-circle arc) = the Slerp path.
  \draw[very thick, blue!70!black] (16:\R) arc (16:76:\R);

  % Central angle Omega.
  \draw[black!70] (16:1.0) arc (16:76:1.0);
  \node at (46:1.34) {$\Omega$};

  % Euclidean chord, its linear interpolant, and the radial projection (= nlerp).
  \draw[dashed, black!45] (u) -- (v);
  \coordinate (m) at ($(u)!0.45!(v)$);
  \fill[black!45] (m) circle (1.4pt);
  \coordinate (nl) at ($(O)!1.18!(m)$);
  \draw[->, black!45] (m) -- (nl);
  \node[black!55, right] at ($(nl)+(0.04,-0.16)$) {$\nlerp$};

  % Slerp point on the geodesic.
  \fill[blue!70!black] (p) circle (1.9pt);
  \node[blue!70!black, above right] at (p) {$\Slerp_\eta(u,v)$};

  % Tangent space at u (perpendicular to Ou; direction 16+90 = 106 deg).
  \draw[red!75!black, thick] ($(u)+(106:2.3)$) -- ($(u)+(106:-1.1)$);
  \node[red!75!black, align=center] at ($(u)+(106:2.62)$) {Tangent at $u$};

  % The geodesic's initial direction, tangent at u, pointing toward v.
  \draw[->, very thick, red!75!black] (u) -- ($(u)+(106:1.7)$);
  \node[red!75!black, left] at ($(u)+(106:0.95)$) {Arc direction};

  % Point labels.
  \node[below right] at (u) {$u$};
  \node[above] at (v) {$v$};
  \node[below left] at (O) {$O$};
\end{tikzpicture}
\caption{Geometry on $\sph^{d-1}$, drawn in the $2$-plane $\mathrm{span}\{u,v\}$ in which the
interpolation lives. The geodesic (great-circle arc, blue) from $u$ to $v$ subtends the central angle
$\Omega=\arccosop\inner{u}{v}$, and $\Slerp_\eta(u,v)$ \eqref{eq:slerp} is the point a fraction
$\eta$ of the way along it. The tangent space at $u$ is shown in this plane as the
red line through $u$, perpendicular to $u$; the red arrow gives the arc's initial direction. The Euclidean chord (grey,
dashed) carries the linear interpolant $(1-\eta)u+\eta v$, which $\nlerp$ renormalizes radially back
onto the sphere (grey arrow); $\nlerp\to\Slerp$ as $\Omega\to0$. At the antipode ($\Omega=\pi$) the
great circle is not unique and $\Slerp$ is undefined.}
\label{fig:sphere}
\end{figure}

